READ-EVAL-PRINT in Parallel and Asynchronous Proof-checking

The LCF tradition of interactive theorem proving, which was started by Milner in the 1970-ies, appears to be tied to the classic READ-EVAL-PRINT-LOOP of sequential and synchronous evaluation of prover commands. We break up this loop and retrofit the read-eval-print phases into a model of parallel and asynchronous proof processing. Thus we explain some key concepts of the Isabelle/Scala approach to prover interaction and integration, and the Isabelle/jEdit Prover IDE as front-end technology. We hope to open up the scientific discussion about non-trivial interaction models for ITP systems again, and help getting other old-school proof assistants on a similar track.

==> eptcsdata.tex <==
\providecommand{\firstpage}{57}
\providecommand{\publicationstatus}{C. Kaliszyk and C. L\"uth (Eds.): 10th International Workshop\\
on User Interfaces for Theorem Provers\\
EPTCS 118, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.118.4}{10.4204/EPTCS.118.4}}
\pdfoutput=1

